Nested Nonparametric Instrumental Variable Regression

Several causal parameters in short panel data models are functionals of a nested nonparametric instrumental variable regression (nested NPIV). Recent examples include mediated, time varying, and long term treatment effects identified using proxy variables. In econometrics, examples arise in triangular simultaneous equations and hedonic price systems. However, it appears that explicit mean square convergence rates for nested NPIV are unknown, preventing inference on some of these parameters with generic machine learning. A major challenge is compounding ill posedness due to the nested inverse problems. To limit how ill posedness compounds, we introduce two techniques: relative well posedness, and multiple robustness to ill posedness. With these techniques, we provide explicit mean square rates for nested NPIV and efficient inference for recently identified causal parameters. Our nonasymptotic analysis accommodates neural networks, random forests, and reproducing kernel Hilbert spaces. It extends to causal functions, e.g. heterogeneous long term treatment effects.

==> 0_commands.tex <==

\addtolength{\oddsidemargin}{-.5in}%
\addtolength{\evensidemargin}{-.1in}%
\addtolength{\textwidth}{1in}%
\addtolength{\textheight}{1.7in}%
\addtolength{\topmargin}{-1in}
\makeatletter
\@ifpackageloaded{caption}{}{\usepackage{caption}}
\AtBeginDocument{%
\ifdefined\contentsname
  \renewcommand*\contentsname{Table of contents}
\else
  \newcommand\contentsname{Table of contents}
\fi
\ifdefined\listfigurename
  \renewcommand*\listfigurename{List of Figures}
\else
  \newcommand\listfigurename{List of Figures}
\fi
\ifdefined\listtablename
  \renewcommand*\listtablename{List of Tables}
\else
  \newcommand\listtablename{List of Tables}
\fi
\ifdefined\figurename
  \renewcommand*\figurename{Figure}
\else
  \newcommand\figurename{Figure}
\fi
\ifdefined\tablename
  \renewcommand*\tablename{Table}
\else
  \newcommand\tablename{Table}
\fi
}
\@ifpackageloaded{float}{}{\usepackage{float}}
\floatstyle{ruled}
\@ifundefined{c@chapter}{\newfloat{codelisting}{h}{lop}}{\newfloat{codelisting}{h}{lop}[chapter]}
\floatname{codelisting}{Listing}
\newcommand*\listoflistings{\listof{codelisting}{List of Listings}}
\makeatother
\makeatletter
\makeatother
\makeatletter
\@ifpackageloaded{caption}{}{\usepackage{caption}}
\@ifpackageloaded{subcaption}{}{\usepackage{subcaption}}
\makeatother


\ifLuaTeX
  \usepackage{selnolig}  % disable illegal ligatures
\fi
\usepackage[]{natbib}
%\bibliographystyle{agsm}
\usepackage{bookmark}

\IfFileExists{xurl.sty}{\usepackage{xurl}}{} % add URL line breaks if available
\urlstyle{same} % disable monospaced font for URLs
\hypersetup{
  pdftitle={Title},
  pdfauthor={Author 1; Author 2},
  pdfkeywords={3 to 6 keywords, that do not appear in the title},
  colorlinks=true,
  linkcolor={blue},
  filecolor={Maroon},
  citecolor={Blue},
  urlcolor={Blue},
  pdfcreator={LaTeX via pandoc}}


\DeclareRobustCommand{\E}{\mathbb{E}}
\DeclareRobustCommand{\N}{\mathbb{N}}
\DeclareRobustCommand{\Q}{\mathbb{Q}}
\DeclareRobustCommand{\H}{\mathbb{H}}
\DeclareRobustCommand{\L}{\mathbb{L}}
\DeclareRobustCommand{\R}{\mathbb{R}}
\DeclareRobustCommand{\P}{\mathbb{P}}
\DeclareRobustCommand{\DS}{\textsc{ds}}
\DeclareRobustCommand{\EXP}{\textsc{exp}}
\DeclareRobustCommand{\OBS}{\textsc{obs}}
\DeclareRobustCommand{\cW}{\mathcal{W}}
\DeclareRobustCommand{\cA}{\mathcal{A}}
\DeclareRobustCommand{\cD}{\mathcal{D}}
\DeclareRobustCommand{\cB}{\mathcal{B}}
\DeclareRobustCommand{\cL}{\mathcal{L}}
\DeclareRobustCommand{\cC}{\mathcal{C}}
\DeclareRobustCommand{\cY}{\mathcal{Y}}
\DeclareRobustCommand{\cS}{\mathcal{S}}
\DeclareRobustCommand{\op}{\text{op}}
\DeclareRobustCommand{\cX}{\mathcal{X}}
\DeclareRobustCommand{\Span}{\text{span}}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareRobustCommand{\d}{\mathrm{d}}

\newcommand{\tr}{\textsc{train}}
\newcommand{\te}{\textsc{test}}

\newcommand{\hpsi}{\hat{\psi}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hsigma}{\hat{\sigma}}
